Quantum-safe Edge Applications: How to Secure Computation in Distributed Computing Systems

The advent of distributed computing systems will offer great flexibility for application workloads, while also imposing more attention to security, where the future advent and adoption of quantum technology can introduce new security threats. For this reason, the Multi-access Edge Computing (MEC) working group at ETSI has recently started delving into security aspects, especially motivated by the upcoming reality of the MEC federation, which involves services made of application instances belonging to different systems (thus, different trust domains). On the other side, Quantum Key Distribution (QKD) can help strengthen the level of security by enabling the exchange of secure keys through an unconditionally secure protocol, e.g., to secure communication between REST clients and servers in distributed computing systems at the edge. In this paper, we propose a technical solution to achieve this goal, building on standard specifications, namely ETSI MEC and ETSI QKD, and discussing the gaps and limitations of current technology, which hamper full-fledged in-field deployment and mass adoption. Furthermore, we provide our look-ahead view on the future of secure distributed computing through the enticing option of federating edge computing domains.

==> newcommands.tex <==

\newcommand{\added}[1]{%
  {\color{blue}#1%
  }%
}
% \renewcommand{\added}[1]{#1}

\newcommand{\removed}[1]{%
  {\color{red}#1%
  }%
}
% \renewcommand{\removed}[1]{}

\newcommand{\highpar}[1]{%
\noindent\colorbox{yellow}{%
\parbox{\dimexpr\linewidth-2\fboxsep}% a box with line-breaks that's just wide enough
{%
#1
}%
}%
}

\setlength{\algomargin}{2em}
\newcommand{\myalgo}[2]{%
\begin{algorithm}%
%\dontprintsemicolon
\include{algorithms/#1}%
\caption{#2}%
\label{algo:#1}%
\end{algorithm}%
}

\newcommand{\mytab}[2]{%
\begin{table}[tbp]%
\caption{#2}%
\centering%
\include{tables/#1}%
\label{tab:#1}%
\end{table}%
}

\newcommand{\mytabfull}[2]{%
\begin{table*}[tbp]%
\caption{#2}%
\centering%
{\small%
\include{tables/#1}%
}%
\label{tab:#1}%
\end{table*}%
}

\newcommand*{\thead}[1]{\multicolumn{1}{c}{\bfseries #1}}

\newcommand{\myfig}[3][width=\columnwidth]{%
\begin{figure}[htbp!]%
\centering%
\includegraphics[#1]{figures/#2}%
\vspace{-1em}%
\caption{#3}%
% \vspace{-1em}%
\label{fig:#2}%
\end{figure}%
}

\newcommand{\myfigdouble}[5][width=\columnwidth]{%
\begin{figure*}[tb]%
\centering%
\includegraphics[#1]{figures/#2}\\
\includegraphics[#1]{figures/#3}%
\caption{#5}%
\label{fig:#4}%
\end{figure*}%
}

\newcommand{\myfigfull}[3][width=\textwidth]{%
\begin{figure*}[tb]%
\centering%
\includegraphics[#1]{figures/#2}%
% \vspace{-1em}%
\caption{#3}%
% \vspace{-1em}%
\label{fig:#2}%
\end{figure*}%
}

\newcommand{\rfig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\ralgo}[1]{Algorithm~\ref{algo:#1}}


\newcommand{\rtab}[1]{Table~\ref{tab:#1}}
\newcommand{\req}[1]{Eq.~(\ref{eq:#1})}
\newtheorem{lemma}{Lemma}

\newenvironment{myinlinelist}%
{%
\begin{enumerate*}[label=(\roman*)]%
}%
{%
\end{enumerate*}%
}

\newenvironment{myitemlist}%
{%
\begin{itemize}[parsep=0em,leftmargin=*,label={--}]%
}%
{%
\end{itemize}%
}

\newenvironment{myenumlist}%
{%
\begin{enumerate}[parsep=0em,leftmargin=*,label=\arabic*.]%
}%
{%
\end{enumerate}%
}

\newcommand{\keypoint}[1]{\noindent\textit{\underline{Key point:} #1}}
\newcommand{\soadiff}[1]{\noindent\textit{\underline{Key difference:} #1}}
